Vector Quantization for Recommender Systems: A Review and Outlook

Vector quantization, renowned for its unparalleled feature compression capabilities, has been a prominent topic in signal processing and machine learning research for several decades and remains widely utilized today. With the emergence of large models and generative AI, vector quantization has gained popularity in recommender systems, establishing itself as a preferred solution. This paper starts with a comprehensive review of vector quantization techniques. It then explores systematic taxonomies of vector quantization methods for recommender systems (VQ4Rec), examining their applications from multiple perspectives. Further, it provides a thorough introduction to research efforts in diverse recommendation scenarios, including efficiency-oriented approaches and quality-oriented approaches. Finally, the survey analyzes the remaining challenges and anticipates future trends in VQ4Rec, including the challenges associated with the training of vector quantization, the opportunities presented by large language models, and emerging trends in multimodal recommender systems. We hope this survey can pave the way for future researchers in the recommendation community and accelerate their exploration in this promising field.

==> Illustration/Plots/paper.tex <==
% \definecolor{c1}{RGB}{252,157,154} % 浅粉红
% \definecolor{c2}{RGB}{249,205,173} % 淡桔黄
% \definecolor{c3}{RGB}{200,200,169} % 淡绿色
% \definecolor{c4}{RGB}{131,175,155} % 淡青绿
% \definecolor{c5}{RGB}{159,129,112} % 淡棕色
% \definecolor{c6}{RGB}{210,180,140} % 淡金色

% \begin{figure}
% \centering
% \resizebox{.7\linewidth}{!}{
% \begin{tikzpicture}
% \begin{axis}[
%     ybar stacked,
%     bar width=15pt,
%     ymin=0,
%     nodes near coords,
%     % enlargelimits=0.15,
%     legend style={
%         at={(0.5,-0.20)},
%         anchor=north,
%         legend columns=3,
%         /tikz/every even column/.append style={column sep=0.5cm}
%     },
%     ylabel={\#Papers},
%     xlabel={Year},
%     symbolic x coords={2004, 2019, 2020, 2021, 2023},
%     xtick=data,
%     x tick label style={rotate=45,anchor=east},
% ]

% \addplot+[ybar,fill=c1,draw=none] plot coordinates {(2004,1) (2019,0) (2020,0) (2021,1) (2023,1)};
% \addplot+[ybar,fill=c2,draw=none] plot coordinates {(2004,0) (2019,1) (2020,1) (2021,0) (2023,1)};
% \addplot+[ybar,fill=c3,draw=none] plot coordinates {(2004,0) (2019,0) (2020,2) (2021,1) (2023,0)};
% \addplot+[ybar,fill=c4,draw=none] plot coordinates {(2004,0) (2019,0) (2020,0) (2021,1) (2023,1)};
% \addplot+[ybar,fill=c5,draw=none] plot coordinates {(2004,0) (2019,0) (2020,0) (2021,0) (2023,1)};
% \addplot+[ybar,fill=c6,draw=none] plot coordinates {(2004,0) (2019,0) (2020,0) (2021,0) (2023,4)};

% \legend{Similarity Search, Space Compression, Time Acceleration, Feature Enhancement, Modality Correlation, Item Tokenization}

% \end{axis}
% \end{tikzpicture}
% }
% \caption{Annual Distribution of VQ Papers Across Different Recommendation Scenarios}
% \end{figure}

